Alya: Towards Exascale for Engineering Simulation Codes

Alya is the BSC in-house HPC-based multi-physics simulation code. It is designed from scratch to run efficiently in parallel supercomputers, solving coupled problems. The target domain is engineering, with all its particular features: complex geome- tries and unstructured meshes, coupled multi-physics with exotic coupling schemes and Physical models, ill-posed problems, flexibility needs for rapidly including new models, etc. Since its conception in 2004, Alya has shown scaling behaviour in an increasing number of cores. In this paper, we present its performance up to 100.000 cores in Blue Waters, the NCSA supercomputer. The selected tests are representative of the engineering world, all the problematic features included: incompressible flow in a hu- man respiratory system, low Mach combustion problem in a kiln furnace and coupled electro-mechanical problem in a heart. We show scalability plots for all cases, discussing all the aspects of such kind of simulations, including solvers convergence.

==> commands.tex <==
% spaces
%\newfont{\toto}        {msbm10}
%\newfont{\coco}        {msam10}
\newcommand{\Real}     {\mbox{\toto R}}

% bold symbols

\newcommand{\bm}[1]    {\mbox{\boldmath{$#1$}}}
\newcommand{\bolda}    {{\bm a}}
\newcommand{\boldd}    {{\bm d}}
\newcommand{\bolde}    {{\bm e}}
\newcommand{\boldf}    {{\bm f}}
\newcommand{\boldbf}   {{\bm F}}
\newcommand{\boldg}    {{\bm g}}
\newcommand{\boldbg}   {{\bm G}}
\newcommand{\boldi}    {{\bm I}}
\newcommand{\boldk}    {{\bm k}}
\newcommand{\boldbm}   {{\bm M}}
\newcommand{\boldn}    {{\bm n}}
\newcommand{\boldo}    {{\bm 0}}
\newcommand{\boldp}    {{\bm p}}
\newcommand{\boldq}    {{\bm q}}
\newcommand{\boldr}    {{\bm r}}
\newcommand{\boldbr}   {{\bm R}}
\newcommand{\bolds}    {{\bm s}}
\newcommand{\boldt}    {{\bm t}}
\newcommand{\boldu}    {{\bm u}}
\newcommand{\boldbu}   {{\bm U}}
\newcommand{\boldv}    {{\bm v}}
\newcommand{\boldw}    {{\bm w}}
\newcommand{\boldbv}   {{\bm V}}
\newcommand{\boldx}    {{\bm x}}
\newcommand{\boldbx}   {{\bm X}}
\newcommand{\boldomega}{{\bm \omega}}
\newcommand{\boldtau}  {{\bm \tau}}
\newcommand{\boldsig}  {{\bm \sigma}}
\newcommand{\boldphi}  {{\bm \phi}}
\newcommand{\boldmu}   {{\bm \mu}}
\newcommand{\bigu}     {{\bm U}}
\newcommand{\bigv}     {{\bm V}}
\newcommand{\defor}    {{\bm \varepsilon}}
\newcommand{\stres}    {{\bm \sigma}}
\newcommand{\shape}    {{\bm N}}

% matrices and vectors

\newcommand{\vectu}    {\mathbf{u}}
\newcommand{\vectf}    {\mathbf{f}}
\newcommand{\vectb}    {\mathbf{b}}
\newcommand{\vecto}    {\mathbf{0}}
\newcommand{\vectp}    {\mathbf{p}}
\newcommand{\vectq}    {\mathbf{q}}
\newcommand{\vectr}    {\mathbf{r}}
\newcommand{\vects}    {\mathbf{s}}
\newcommand{\vectt}    {\mathbf{t}}
\newcommand{\vectv}    {\mathbf{v}}
\newcommand{\vectw}    {\mathbf{w}}
\newcommand{\vectx}    {\mathbf{x}}
\newcommand{\vecty}    {\mathbf{y}}
\newcommand{\vectz}    {\mathbf{z}}

\newcommand{\matra}    {\mathbf{A}}
\newcommand{\matrc}    {\mathbf{C}}
\newcommand{\matrd}    {\mathbf{D}}
\newcommand{\matrg}    {\mathbf{G}}
\newcommand{\matrl}    {\mathbf{L}}
\newcommand{\matrm}    {\mathbf{M}}
\newcommand{\matro}    {\mathbf{0}}
\newcommand{\matrp}    {\mathbf{P}}
\newcommand{\matrq}    {\mathbf{Q}}
\newcommand{\matrs}    {\mathbf{S}}
\newcommand{\matru}    {\mathbf{U}}
\newcommand{\matrwaa}  {\mathbf{WA1}}
\newcommand{\matrwab}  {\mathbf{WA2}}

% subdomains definitions

\newcommand{\A}{3}
\newcommand{\B}{4}
\newcommand{\C}{5}
\newcommand{\1}{1}
\newcommand{\2}{2}
\newcommand{\ga}{a}
\newcommand{\gb}{b}

% Physical parameters

\newcommand{\s}{s}
\newcommand{\sou}{s}
\newcommand{\adv}{\mbox{\boldmath $a$}}
\newcommand{\dif}{\varepsilon}
\newcommand{\dis}{D}

